Better Source, Better Flow: Learning Condition-Dependent Source Distribution for Flow Matching

Flow matching has recently emerged as a promising alternative to diffusion-based generative models, particularly for text-to-image generation. Despite its flexibility in allowing arbitrary source distributions, most existing approaches rely on a standard Gaussian distribution, a choice inherited from diffusion models, and rarely consider the source distribution itself as an optimization target in such settings. In this work, we show that principled design of the source distribution is not only feasible but also beneficial at the scale of modern text-to-image systems. Specifically, we propose learning a condition-dependent source distribution under flow matching objective that better exploit rich conditioning signals. We identify key failure modes that arise when directly incorporating conditioning into the source, including distributional collapse and instability, and show that appropriate variance regularization and directional alignment between source and target are critical for stable and effective learning. We further analyze how the choice of target representation space impacts flow matching with structured sources, revealing regimes in which such designs are most effective. Extensive experiments across multiple text-to-image benchmarks demonstrate consistent and robust improvements, including up to a 3x faster convergence in FID, highlighting the practical benefits of a principled source distribution design for conditional flow matching.

==> tables/large_scale.tex <==
\begin{wraptable}{r}{0.98\textwidth}
\vspace{-1em}
\centering

\begin{minipage}[t]{0.52\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
\textbf{Method} & \textbf{FID~$\downarrow$} & \textbf{CLIP~$\uparrow$} & 
\textbf{IS~$\uparrow$} & \textbf{FDD~$\downarrow$} &
\textbf{VQAScore~$\uparrow$}\\
\midrule
Standard FM & 2.925 & 0.3396 & 187.0 & 69.37 & -- \\
\midrule
CrossFlow~\cite{liu2025crossflow} & 2.957 & 0.3301 & -- & -- & -- \\
C$^2$OT~\cite{cheng2025c2ot} & 3.365 & 0.3406 & -- & -- & -- \\
CPD~\cite{issachar2025designing} & -- & -- & -- & -- & -- \\
CAR-Flow~\cite{chen2025carflow} & 2.929 & 0.3408 & 192.8 & 66.38 & -- \\
\rowcolor{blue!10}
\textbf{CSFM (Ours)} & \textbf{2.453} & \textbf{0.3433} & \textbf{203.7} & \textbf{54.00} & \textbf{0.5338} \\
\bottomrule
\end{tabular}}
\end{minipage}
\hfill
\begin{minipage}[t]{0.42\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|cc}
\toprule
\textbf{Model} & \textbf{\#Params} & \textbf{GenEval} & \textbf{DPG-Bench} \\
\midrule
\multirow{2}{*}{BLIP3o~\cite{chen2025blip3o}} & 4B & 0.81 & 79.36 \\
& 8B & 0.84 & 81.60 \\
\multirow{2}{*}{Sana~\cite{xie2024Sana}} & 0.6B & 0.64 & 83.60 \\
& 1.6B & 0.66 & 84.80 \\
\midrule
Standard FM & 1.3B & 0.77 & 78.31 \\
\rowcolor{blue!10}
\textbf{CSFM (Ours)} & 1.3B & \textbf{0.80} & \textbf{81.11} \\
\bottomrule
\end{tabular}}
\end{minipage}

\caption{\textbf{Comparison to prior methods and large-scale text-to-image evaluation.}
Left: condition-aware coupling/source methods on ImageNet 256$\times$256. 
Right: GenEval and DPG-Bench results.}
\label{tab:combined_results}
\vspace{-1.5em}
\end{wraptable}

% \begin{table}[t]
% \centering
% \caption{\textbf{Large-scale text-to-image evaluation.} Results on GenEval and DPG-Bench. We report standard FM and CSFM with UnifiedNextDiT (1.3B), together with results from prior work that evaluate the same model families at different parameter scales, to contextualize the magnitude of performance gains at this scale.
% }
% \vspace{0.5em}
% \resizebox{0.44\textwidth}{!}{
% \begin{tabular}{l|c|cc}
%         \toprule
%         \textbf{Model} & \textbf{\#Params} & \textbf{GenEval} & \textbf{DPG-Bench}  \\
%         \midrule
%         \midrule
%         \multirow{2}{*}{BLIP3o~\cite{chen2025blip3o}} & 4B & 0.81 & 79.36 \\
%         & 8B & 0.84 & 81.60 \\
%         \multirow{2}{*}{Sana~\cite{xie2024Sana}} & 0.6B & 0.64 & 83.60 \\
%         & 1.6B & 0.66 & 84.80 \\
%         % \multirow{2}{*}{Janus Pro~\cite{chen2025janus}} & 1B & 0.73 & 82.63 \\
%         % & 7B & 0.80 & 84.19  \\
%         \midrule
%         \multicolumn{1}{c|}{Standard FM} & 1.3B & 0.77 & 78.31  \\
%         \rowcolor{blue!10} \multicolumn{1}{c|}{\textbf{CSFM (Ours)}} & 1.3B & \textbf{0.80} & \textbf{81.11}   \\
%         \bottomrule
% \end{tabular}}
% \label{tab:scale_results}
% \vspace{-13pt}
% \end{table}

% }
% \subcaption{Condition Drop}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.325\textwidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{0.38mm}{
% \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Model Size} & \textbf{IS}↑ & \textbf{FID}↓ & \textbf{sFID}↓ & \textbf{Pr.}↑ & \textbf{Rc.}↑ \\
%         \midrule
%         SiT-B & 27.5 & 49.50 & 7.00 & 0.46 & 0.59 \\
%         \rowcolor{green!10} \textbf{+iREPA} & \textbf{34.1} & \textbf{43.37} & \text{7.87} & \textbf{0.50} & \textbf{0.60} \\
%         \midrule
%         SiT-L & 55.7 & 24.10 & 6.25 & 0.62 & 0.60 \\
%         \rowcolor{green!10} \textbf{+iREPA} & \textbf{66.9} & \textbf{20.28} & \textbf{6.14} & \textbf{0.63} & \textbf{0.62} \\
%         \midrule
%         SiT-XL & 70.3 & 19.06 & 5.83 & 0.65 & 0.61 \\
%         \rowcolor{green!10} \textbf{+iREPA} & \textbf{77.9} & \textbf{16.96} & \text{6.26} & \textbf{0.66} & \textbf{0.61} \\
%         \bottomrule
% \end{tabular}
% }
% \subcaption{Model size}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.325\textwidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{0.38mm}{
% \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Aln. Depth} & \textbf{IS}↑ & \textbf{FID}↓ & \textbf{sFID}↓ & \textbf{Pr.}↑ & \textbf{Rc.}↑ \\
%         \midrule
%         Layer 4 & 28.1 & 49.0 & 6.83 & 0.46 & 0.60 \\
%         \rowcolor{cyan!10} \textbf{+iREPA} & \textbf{41.7} & \textbf{36.0} & \textbf{6.61} & \textbf{0.52} & \textbf{0.62} \\
%         \midrule
%         Layer 6 & 26.9 & 50.6 & 7.00 & 0.46 & 0.59 \\
%         \rowcolor{cyan!10} \textbf{+iREPA} & \textbf{42.4} & \textbf{35.3} & \textbf{6.90} & \textbf{0.53} & \textbf{0.62} \\
%         \midrule
%         Layer 8 & 24.7 & 54.8 & 7.35 & 0.44 & 0.58 \\
%         \rowcolor{cyan!10} \textbf{+iREPA} & \textbf{38.3} & \textbf{38.9} & \textbf{7.19} & \textbf{0.51} & \textbf{0.62} \\
%         \bottomrule
% \end{tabular}
% }
% \subcaption{Encoder depth (SiT-B/2)}
% \end{minipage}

% \caption{\textbf{Variation in training settings.} We find that iREPA leads to consistent gains over baseline REPA across diverse training settings. Unless otherwise specified all results are reported using Dinov2 as encoder, SiTXL/2, 100K steps and vanilla-REPA as baseline.}
% \label{tab:model_encoder_depth}
% \end{table*}
